Mitigating Spurious Correlations in Multi-modal Models during Fine-tuning

Spurious correlations that degrade model generalization or lead the model to be right for the wrong reasons are one of the main robustness concerns for real-world deployments. However, mitigating these correlations during pre-training for large-scale models can be costly and impractical, particularly for those without access to high-performance computing resources. This paper proposes a novel approach to address spurious correlations during fine-tuning for a given domain of interest. With a focus on multi-modal models (e.g., CLIP), the proposed method leverages different modalities in these models to detect and explicitly set apart spurious attributes from the affected class, achieved through a multi-modal contrastive loss function that expresses spurious relationships through language. Our experimental results and in-depth visualizations on CLIP show that such an intervention can effectively i) improve the model's accuracy when spurious attributes are not present, and ii) directs the model's activation maps towards the actual class rather than the spurious attribute when present. In particular, on the Waterbirds dataset, our algorithm achieved a worst-group accuracy 23% higher than ERM on CLIP with a ResNet-50 backbone, and 32% higher on CLIP with a ViT backbone, while maintaining the same average accuracy as ERM.

==> 3_method.tex <==
\section{Spurious-aware Contrastive Language Image Fine-tuning}
\label{sec:method}


\paragraph{Background.}  Contrastive Language-Image Pretraining (CLIP) learns from millions of image caption pairs, by maximizing the agreement between representations of every image and the representations of its corresponding caption. 
Specifically, the CLIP architecture consists of (i) an image encoder network, %
(ii) a text encoder network, %
and (iii) a contrastive objective that pulls the embeddings of
every image and its corresponding caption together while pushing apart embeddings of the image from other captions in the same minibatch.
Formally, for a minibatch of $N$ image-captions pairs $\{I_j,T_j\}_{j=1}^N$, and their encoded embeddings $\{I_j^e,T_j^e\}_{j=1}^N$, the CLIP loss is defined as follows:
\begin{align}
    \mathcal{L}_{\text{CLIP}}
    =&-\frac{1}{2}\E_{(I_i,T_i)} \log \left [ \frac{e^{\left<I_j^e,T_j^e\right>/\tau}}{\sum_{k=1}^N e^{\left<I_j^e,T_k^e\right>/\tau} } \right] \label{eq:cliploss}\\
    &-\frac{1}{2}\E_{(I_i,T_i)} \log \left [ \frac{e^{\left<I_k^e,T_k^e\right>/\tau}}{\sum_{j=1}^N e^{\left<I_j^e,T_k^e\right>/\tau} } \right],\nonumber   
\end{align}
where $\left<.,.\right>$ represents the inner product, and $\tau$ is a trainable temperature parameter.
For finetuning CLIP on a dataset of images and their labels, such as Waterbirds, the labels are replaced in the engineered prompt templates, such as
``A photo of a \{label\}", 
``A photo of a \{label\}, a type of bird.”, etc. Then, the loss is minimized on the images paired with templates built with image labels.


 
For a given spurious attribute (e.g. water or land background in the Waterbirds dataset), we will use the following losses to eliminate the spurious correlation during fine-tuning. Please note that the contrastive losses below use the class information to pull together representations of examples from the same class label, and push away representations of examples from different class labels. The spurious losses use the spurious attribute detected in the spurious correlation detection stage (Section~\ref{sec:detection}) to pull together representations of examples with the same spurious attribute (e.g. attribute present) and push away representations of examples with a different spurious attribute (e.g. attribute absent). 



\paragraph{Contrastive Image Loss}
The first term is a contrastive image loss which pulls together image representations of a class, and pushes away image representations of different classes in the vision model.
Let $\{(I_p,T_p)\}_{p=1}^P$ be the set of examples in the minibatch with the \textbf{same label} as example $(I_i,T_i)$, i.e., $T_i\!=\!T_p$, and $\{(I_q,T_q)\}_{q=1}^Q$ be the set of examples with a \textbf{different label}. Then the contrastive image loss is defined as:
\begin{align}
    \mathcal{L}_{vc}\!=\!-\hspace{-6mm}\E_{\substack{(I_i,T_i),\\ \{(I_p,T_p)\}_{p=1}^P\\ \{(I_q,T_q)\}_{q=1 }^Q}} 
    \!\!\!\left[\log \frac{ e^{\left<I_i^e,I_p^e\right>/\tau}}{\sum_{p=1}^P e^{\left<I_i^e,I_p^e\right>/\tau}+\sum_{q=1}^Q e^{\left<I_i^e,I_q^e\right>/\tau}} \right]\!\! \nonumber
\end{align}

\paragraph{Contrastive Language Loss}
The second term is a contrastive language loss which pulls together language representations of templates of a class in the language model, and pushes away language representations of different classes.
Let $\{(I_p,T_p)\}_{p=1}^P$ be the set of examples in the minibatch with the \textbf{same label} as example $(I_i,T_i)$, i.e., $T_i\!=\!T_p$, but with different templates. Let $\{(I_q,T_q)\}_{q=1}^Q$ be the set of examples in the minibatch with a \textbf{different label}. Then the contrastive language loss is defined as:
\begin{align}
    \mathcal{L}_{lc}\!=\!-\hspace{-6mm}\E_{\substack{(I_i,T_i),\\ \{(I_p,T_p)\}_{p=1}^P\\ \{(I_q,T_q)\}_{q=1 }^Q}} 
    \!\!\!\left[\log \frac{ e^{\left<T_i^e,T_p^e\right>/\tau}}{\sum_{p=1}^P e^{\left<T_i^e,T_p^e\right>/\tau}+\sum_{q=1}^Q e^{\left<T_i^e,T_q^e\right>/\tau}} \right]\!\! \nonumber
\end{align}


\paragraph{Spurious Image Loss}
The third term is a spurious contrastive image loss which pulls together image representations of each group of examples in a class, and pushes away image representations of different groups of examples. For example, it pulls together images of waterbirds with water background, and pulls them away from images of waterbirds with land background and from landbird images with water or land background.

Assume $\{(I_p,T_p)\}_{p=1}^P$ is the set of images in the minibatch with the \textbf{same spurious attribute} as example $(I_i,T_i)$, and $\{(I_q,T_q)\}_{q=1}^Q$ is the set of examples with a \textbf{different spurious attribute} than example $(I_i,T_i)$.  A different spurious attribute here could also mean that the spurious attribute is absent. Then, the spurious image loss is defined as:
\begin{align}
    \mathcal{L}_{vs}\!=\!-\hspace{-5mm} \E_{\substack{(I_i,T_i),\\ \{(I_p,T_p)\}_{p=1}^P\\ \{(I_q,T_q)\}_{q=1 }^Q}} 
    \!\!\!\left[
    \log \frac{e^{ \left<I_{i}^e,I_{p}^e\right>/\tau}}{\sum_{p=1}^P e^{\left<I_{i}^e,I_{p}^e\right>/\tau}\!\!+\!\sum_{q=1}^Q e^{\left<I_{i}^e,I_{q}^e\right>/\tau}}\! 
    \right]\!\! \nonumber
\end{align}

\paragraph{Spurious Language Loss}
The last term is a spurious contrastive language loss which pulls together language representations of each group of examples in a class, and pushes away language representations of different groups of examples.
Assume $\{(I_p,T_p)\}_{p=1}^P$ is the set of examples in the minibatch with the \textbf{same spurious attribute} with example $(I_i,T_i)$, and $\{(I_q,T_q)\}_{q=1}^Q$ is the set of examples with a \textbf{different spurious attribute} in the minibatch. Note that, a different spurious attribute here could also mean that a spurious attribute is absent. Then, the spurious language loss is defined as:
\begin{align}
    \mathcal{L}_{ls}\!=\!\!-\hspace{-5mm} \E_{\substack{(I_i,T_i),\\ \{(I_p,T_p)\}_{p=1}^P\\ \{(I_q,T_q)\}_{q=1 }^Q}} 
    \!\!\!\left[
    \log \frac{e^{ \left<T_{i}^e,T_{p}^e\right>/\tau}}{\sum_{p=1}^P e^{\left<T_{i}^e,T_{p}^e\right>/\tau}\!\!+\!\sum_{q=1}^Q e^{\left<T_{i}^e,T_{q}^e\right>/\tau}} 
    \!\right]\!\! \nonumber
\end{align}









The final loss is the sum of all the terms above:
\begin{equation}
\mathcal{L}=\mathcal{L}_{\text{CLIP}}+\mathcal{L}_{vc}+\mathcal{L}_{lc}+\mathcal{L}_{vs}+\mathcal{L}_{ls}.
\end{equation}

In practice, either $\mathcal{L}_{vs}$ or $\mathcal{L}_{ls}$ can be combined with $\mathcal{L}_{lc}$ to effectively eliminate the spurious correlation. If spurious attribute annotation labels are available, one can use $\mathcal{L}_{vs}$. If spurious attribute annotation labels are not available $\mathcal{L}_{ls}$ can provide a good separation between groups in different classes. In all experiments reported hereafter we show results for both, and the ablation study in Section~\ref{sec:loss-ablation} details the tradeoffs between these and other choices.


From an implementation perspective, all language-related losses could be implemented across examples or templates. Our implementation follows a template-based approach.

\begin{figure*}[ht]
\vskip 0.2in
\begin{center}
\centerline{\includegraphics[width=.8\textwidth]{figures/spurious-diagram.png}}
\caption{Spurious correlation detection based on attributes from an open-vocabulary detector and accuracy discrepancy scores of the model between examples when the spurious attribute is present or absent. }
\label{fig:detection-diagram}
\end{center}
\vskip -0.2in
\end{figure*}

\section{Spurious Correlation Detection}
\label{sec:detection}
This section introduces our pipeline for detecting and evaluating spurious correlations learned by a pretrained model. While we apply this pipeline to CLIP models in this work, it can be generalized to other pretrained models as well. The approach closely follows previously discussed techniques~\cite{singlaCVPR2021,nushi2018towards} but relies on automatically generated annotations for attributes.

\subsection{Methodology}


For any given fine-tuning dataset, we are interested in knowing whether CLIP (or any other pretrained models) has learned any spurious correlations for the classes in the dataset. According to the definition of spurious attributes introduced in \cref{sec:method}, models that have learned a certain spurious correlation usually show better performance (e.g., higher classification accuracy) on examples with that spurious attribute. For example, a model that majorly relies on the presence of an emergency vehicle to detect an accident, would have a lower accuracy in detecting accidents when there are no emergency vehicles around. 

We use the pipeline depicted in Figure~\ref{fig:detection-diagram} to (1) find such spurious attributes for a class of interest if the spurious attributes are unknown, and (2) measure how much each spurious attribute negatively affects the model. 

\paragraph{Spurious Detection.} For the case where the spurious attribute is unknown, we first use an open-vocabulary detector, OWL-ViT \cite{minderer2022simple}, to detect potential spurious attributes for examples in the fine-tuning data. We use the synsets of object names in Visual Genome \cite{krishnavisualgenome} as our list of attributes to detect after removing objects that are classes of the fine-tuning data. 

\paragraph{Spurious Evaluation.} We define $\delta(\mathcal{D}, s)$ as the model accuracy discrepancy between examples in dataset $\mathcal{D}$ with the attribute $s$ and those without it.  
\begin{align}
\delta(\mathcal{D},s) = acc(\mathcal{D} | s=1) - acc(\mathcal{D} | s=0)
\end{align}

Attributes detected in the fine-tuning dataset can then be ranked by their accuracy discrepancy scores. The higher the discrepancy, the more this attribute could harm the generalization performance of the pretrained model. Since model failure modes and in particular spurious correlations are often specific to the class~\cite{nushi2018towards}, for the ImageNet studies we compute and sort the discrepancy scores per class. While the drop in accuracy with the absence of the spurious attributes are good indicators of spurious correlations, such drops may also happen for healthy attributes that are part of the class definition (e.g., the yellow color for taxi cabs albeit not all taxis are yellow).

Thus, for practical usages of our approach, we imagine this step to involve some miminal human investigation from either domain experts or ML practitioners to judge whether the attribute is healthy or a potential spurious correlation. Humans can make this call based on their knowledge about the domain or one of the vision interpretability techniques (e.g, Grad-CAM, Integrated Gradients etc.). Nevertheless, this kind of supervision is considerably more lightweight than annotating attributes or even manually inspecting individual examples.\cref{tab:imagenet_spurious_correlations} shows several examples of previously unknown spurious correlations we found for CLIP in the ImageNet dataset. 


